CLIP-Dissect: Automatic Description of Neuron Representations in Deep Vision Networks

In this paper, we propose CLIP-Dissect, a new technique to automatically describe the function of individual hidden neurons inside vision networks. CLIP-Dissect leverages recent advances in multimodal vision/language models to label internal neurons with open-ended concepts without the need for any labeled data or human examples. We show that CLIP-Dissect provides more accurate descriptions than existing methods for last layer neurons where the ground-truth is available as well as qualitatively good descriptions for hidden layer neurons. In addition, our method is very flexible: it is model agnostic, can easily handle new concepts and can be extended to take advantage of better multimodal models in the future. Finally CLIP-Dissect is computationally efficient and can label all neurons from five layers of ResNet-50 in just 4 minutes, which is more than 10 times faster than existing methods. Our code is available at https://github.com/Trustworthy-ML-Lab/CLIP-dissect. Finally, crowdsourced user study results are available at Appendix B to further support the effectiveness of our method.

==> Table/method_strenghts.tex <==
\begin{table}[]
\caption{Comparison of existing automated neuron labeling methods and whether they have certain desirable properties. * Depends on choice of comparison function $\textit{dist}$. \lily{need to update this table, and what's the column: describe more than top few images?}}
\centering
\scalebox{0.88}{
\begin{tabular}{@{}llllllll@{}}
\toprule
\begin{tabular}[c]{@{}l@{}}Property / \\ Method \end{tabular} & \begin{tabular}[c]{@{}l@{}}Computa-\\ tionally \\ Efficient\end{tabular} & \begin{tabular}[c]{@{}l@{}}Unrest- \\ ricted \\ concepts\end{tabular} & \begin{tabular}[c]{@{}l@{}}Does not \\ binarize \\ activations\end{tabular} & \begin{tabular}[c]{@{}l@{}}Describes \\ more than \\ top few \\ images\end{tabular} & \begin{tabular}[c]{@{}l@{}}Uses spatial \\ information \\ of neuron \\ activations\end{tabular} & \begin{tabular}[c]{@{}l@{}}Generative \\ natural \\ language \\ descriptions\end{tabular} & \begin{tabular}[c]{@{}l@{}}Generalizes \\ to different \\ vision tasks\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Network \\ Dissection \\ (\cite{netdissect2017})\end{tabular} & \textbf{Yes} & No & No & \textbf{Yes} & \textbf{Yes} & No & No \\ \midrule
\begin{tabular}[c]{@{}l@{}}Compositional \\ Explanations \\ (\cite{mu2020compositional}) \end{tabular} & No & No & No & \textbf{Yes} & \textbf{Yes} & No & No \\ \midrule
\begin{tabular}[c]{@{}l@{}}MILAN \\ (\cite{hernandez2022natural}) \end{tabular} & ? & \textbf{Yes} & No & No & \textbf{Yes} & \textbf{Yes} & ? \\ \midrule
\begin{tabular}[c]{@{}l@{}}\algoname \\ \textbf{(Ours)} \end{tabular}  & \textbf{Yes} & \textbf{Yes} & \textbf{Yes*} & \textbf{Yes*} & No & No & \textbf{Yes} \\ \bottomrule
\end{tabular}}

\label{tab:method_strengths}
\end{table}
